The Second DiCOVA Challenge: Dataset and performance analysis for COVID-19 diagnosis using acoustics

The Second Diagnosis of COVID-19 using Acoustics (DiCOVA) Challenge aimed at accelerating the research in acoustics based detection of COVID-19, a topic at the intersection of acoustics, signal processing, machine learning, and healthcare. This paper presents the details of the challenge, which was an open call for researchers to analyze a dataset of audio recordings consisting of breathing, cough and speech signals. This data was collected from individuals with and without COVID-19 infection, and the task in the challenge was a two-class classification. The development set audio recordings were collected from 965 (172 COVID-19 positive) individuals, while the evaluation set contained data from 471 individuals (71 COVID-19 positive). The challenge featured four tracks, one associated with each sound category of cough, speech and breathing, and a fourth fusion track. A baseline system was also released to benchmark the participants. In this paper, we present an overview of the challenge, the rationale for the data collection and the baseline system. Further, a performance analysis for the systems submitted by the $16$ participating teams in the leaderboard is also presented.

==> plot_baseline_diag_val_ROC.tex <==
\begin{tikzpicture}
% ----- row 1: put the images
\node[inner sep=0pt,anchor=center] (main_fig) at (2,10) % {x,y} from left corner in an imagined grid
{\includegraphics[width=5cm,height=7cm]{figures/DiCOVA2Baseline.png}};

\node[inner sep=0pt,anchor=center] (main_fig) at (10,10) % {x,y} from left corner in an imagined grid
{\includegraphics[width=7cm,height=7cm]{figures/SecondDiCOVA_basline_val_auc_roc.pdf}};


% ----- put axis labels
\node[font=\fontsize{8}{6}\selectfont,rotate=0,anchor=center] at (2,6.15) (l1) {(a)};
\node[font=\fontsize{8}{6}\selectfont,rotate=0,anchor=center] at (10,6.15) (l1) {(b)};

\end{tikzpicture}

==> table_perfm_test.tex <==
\begin{table}[]
\centering
\rowcolors{2}{white}{gray!10}
\begin{tabular}{@{}llcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Test}} &  & \multicolumn{4}{c}{\textbf{AUC-ROC Performance (in \%)}} \\ \cmidrule(l){3-6} 
 &  & \textbf{Breathing} & \textbf{Cough} & \textbf{Speech} & \textbf{Fusion} \\ \midrule
Blind &  & 84.50 & 74.89 & 84.26 & 84.70 \\
\bottomrule
\end{tabular}
\caption{Baseline System performance on the blind test set.}
\label{table:perfm_test}
\end{table}
